Piecewise semi-ellipsoidal control invariant sets

Computing control invariant sets is paramount in many applications. The families of sets commonly used for computations are ellipsoids and polyhedra. However, searching for a control invariant set over the family of ellipsoids is conservative for systems more complex than unconstrained linear time invariant systems. Moreover, even if the control invariant set may be approximated arbitrarily closely by polyhedra, the complexity of the polyhedra may grow rapidly in certain directions. An attractive generalization of these two families are piecewise semi-ellipsoids. We provide in this paper a convex programming approach for computing control invariant sets of this family.

==> Makefile <==
# You can change the pdf viewer to your preferred
# one by commenting every line beginning by
# `PDFVIEWER' except the one with your pdf viewer
PDFVIEWER=evince # GNOME
#PDFVIEWER=okular # KDE
#PDFVIEWER=xpdf # lightweight
#PDFVIEWER=xdg-open # Default pdf viewer - GNU/Linux
#PDFVIEWER=open # Default pdf viewer - Mac OS
MAIN_NAME=2020_PieceQuad-paper
PDF_NAME=$(MAIN_NAME).pdf

# You want latexmk to *always* run, because make does not have all the info.
.PHONY: $(PDF_NAME) clean show release

# If you want the pdf to be opened by your preferred pdf viewer
# after `$ make', comment the following line and uncomment the
# line after
#default: all
default: show

all: $(PDF_NAME)

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interactive=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

# Other depences are gessed automatically by latexmk
# see http://tex.stackexchange.com/questions/40738/how-to-properly-make-a-latex-project
$(PDF_NAME): $(MAIN_NAME).tex
	latexmk -pdf -pdflatex="pdflatex -shell-escape -enable-write18" \
	  -use-make $(MAIN_NAME).tex

clean:
	latexmk -CA
	$(RM) $(MAIN_NAME).bbl

show: $(PDF_NAME)
	$(PDFVIEWER) $(PDF_NAME) 2> /dev/null &

publish: $(PDF_NAME)
	cp $(PDF_NAME) ~/Dropbox/Research/$(NAME)

release:
	if [ -a config.yml ] ; \
	then \
		python3 ~/git/smartcp/smartcp.py --google-drive -vvvvv config.yml ; \
	else \
		cp $(MAIN_NAME).pdf ~/gdrive/Research/$(TYPE)/$(NAME).pdf; \
		drive push ~/gdrive/Research/$(TYPE)/$(NAME).pdf; \
	fi;
ifdef PDFNAME
	if ! [ -a config.yml ] ; \
	then \
		cp $(MAIN_NAME).pdf "/home/blegat/gdrive/Research benoit et raph/Final versions/$(PDFNAME).pdf"; \
		drive push "/home/blegat/gdrive/Research benoit et raph/Final versions/$(PDFNAME).pdf"; \
	fi;
endif

